Convergence of regularized particle filters for stochastic reaction networks

Filtering for stochastic reaction networks (SRNs) is an important problem in systems/synthetic biology aiming to estimate the state of unobserved chemical species. A good solution to it can provide scientists valuable information about the hidden dynamic state and enable optimal feedback control. Usually, the model parameters need to be inferred simultaneously with state variables, and a conventional particle filter can fail to solve this problem accurately due to sample degeneracy. In this case, the regularized particle filter (RPF) is preferred to the conventional ones, as the RPF can mitigate sample degeneracy by perturbing particles with artificial noise. However, the artificial noise introduces an additional bias to the estimate, and, thus, it is questionable whether the RPF can provide reliable results for SRNs. In this paper, we aim to identify conditions under which the RPF converges to the exact filter in the filtering problem determined by a bimolecular network. First, we establish computationally efficient RPFs for SRNs on different scales using different dynamical models, including the continuous-time Markov process, tau-leaping model, and piecewise deterministic process. Then, by parameter sensitivity analyses, we show that the established RPFs converge to the exact filters if all reactions leading to an increase of the molecular population have linearly growing propensities and some other mild conditions are satisfied simultaneously. This ensures the performance of the RPF for a large class of SRNs, and several numerical examples are presented to illustrate our results.

==> proof2.tex <==
\section{The proof of \cref{thm main}}\label{section proof}

\textcolor{blue}{
We first outline the strategy to prove our main result.
Note that the error of a particle filter comes from model reduction, finite sampling, resampling, and artificial evolution.
Here, we can easily analyze the error introduced by model reduction using techniques in \cite{calzolari2006approximation,fang2021stochastic} and the error caused by finite sampling and resampling using the tools in  \cite{del2000branching,crisan2001particle,bain2008fundamentals}.
Therefore, the key to proving our main result lies in the analysis of artificial evolution. 
In this appendix, we show that the error caused by artificial evolution is of the order $\frac{1}{\sqrt{M}}$ (where $M$ is the particle population) by the the parameter sensitivity analysis, and, thus, this error vanishes as the particle population goes to infinite. 
Finally, by combing all the error analysis results, we can prove the main theorem. 
} 

\textcolor{blue}{
To make the idea more explicit, we formulate the proof outline as follows.
First, since the model reduction is not the key factor in this proof, we simplify the notation by removing the superscript that specifies the dynamical model applied.
Specifically, for a given RPF constructed in \Cref{def RPFs for SCRNs}, we term
\begin{equation}\label{eq. notations}
	\begin{array}{lcl}
	\bar \pi_{M,t_i}(\phi) & \text{as} & 
	 \text{the particle filter }\bar \pi^{N,\gamma_1}_{M,t_i}(\phi),~ \bar \pi^{N,\gamma_1,\tau}_{M,t_i}(\phi), ~\text{or} ~\bar \pi^{N,\gamma_1,H}_{M,t_i}(\phi), \\
	 \hat \pi_{M,t_i}(\phi) &\text{as} & \text{the estimate of the function $\phi$ based on resampled particles} \\
	 && (\hat \pi_{M,t_i}(\phi) \triangleq \frac{1}{M}{\sum_{j=1}^{M} \phi(\hat \kappa_j(t_i), \bar x_j(t_i))}),\\
	 \tilde \pi_{M,t_i}(\phi) &\text{as} &\text{the estimate of the function $\phi$ based on artificially perturbed} \\
	 && \text{particles } (\tilde \pi_{M,t_i}(\phi) \triangleq \frac{1}{M}\sum_{j=1}^{M}  \phi(\bar \kappa_j(t_i), \bar x_j(t_i))),\\
	 \pi_{t_{i+1}}(\phi) &\text{as} & \text{the exact filter $\pi^{N,\gamma_{1}}_{t_{i+1}}(\phi)$},\\
	 K_t & \text{as} & \text{the transition kernel of the applied dynamical system} \\ &&\text{(the CTMC, tau-leaping model, or PDMP)},\\
	 K^{N,\gamma_1}_t & \text{as} & \text{the transition kernel of the full model}\\
	 Y(t_i) &\text{as} & \text{the observation $Y^{N,\gamma_{1}}(t_{i})$},\\
	 \Delta t_i &\text{as} & t_{i+1}-t_{i}.
	\end{array}
\end{equation}
With these notations, we can decompose the error between the RPF $\bar \pi_{M,t_{i+1}} (\phi)$ and the exact filter $\pi_{t_{i+1}}(\phi)$ as follows.
\begin{align}\label{eq. bias caused by artificial evolution}
	\bar \pi_{M,t_{i+1}} (\phi) - \pi_{t_{i+1}}(\phi) 
	&= \bar \pi_{M,t_{i+1}} (\phi)  - \frac{\pi_{t_{i}}( K^{N,\gamma_1}_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}{\pi_{t_{i}}( K^{N,\gamma_1}_{\Delta t_i} \ell _{Y(t_{i+1})})} \notag\\
	&=\underbrace{\left(\bar \pi_{M,t_{i+1}} (\phi)- \frac{\tilde \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}{Z_{t}} \right)}_\text{the error caused by finite sampling}  \\
	&\quad+\frac{1}{Z_t} 
	\underbrace{\Big({\tilde \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)} -
	{\hat \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)} \Big)}_\text{the error caused by the artificial evolution}
	\notag\\
	&\quad+\frac{1}{Z_t}
		\underbrace{\Big(
		{\hat \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}
	- {\bar \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}
	\Big)}_\text{the error caused by resampling} \notag\\
	&\quad+\frac{1}{Z_t}
    \underbrace{\Big(
	{\bar \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}
	-  { \pi_{t_{i}}( K^{N,\gamma_1}_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}
	\Big)}_\text{the error of the particle filter at $t_i$} \notag 
%		&\quad+\frac{1}{Z_t}
%	\underbrace{\Big(
%	{ \pi_{M,t_{i}} ( K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}
%	-  {\pi_{t_{i}}( K^{N,\gamma_1}_{\Delta t_i} \ell _{Y(t_{i+1})}\phi)}
%	\Big)}_\text{the error caused by model reduction} \notag
\end{align}
where the first equality follows from the recursive formulas \eqref{eq. recurssive expression 1} and \eqref{eq. recurssive expression 2}, the term $\ell_{Y(t_{i+1})} $ is the likelihood function (see \eqref{eq. recurssive expression 2} and the text below), and $Z_{t}=\pi_{t_{i}}( K^{N,\gamma_1}_{\Delta t_i} \ell _{Y(t_{i+1})})$.
Here, the error caused by model reduction is hidden in the last term, because the transition kernels in the last line represent the reduced model and the full model, respectively, (see \eqref{eq. notations}).
Also, we note that both the likelihood function and $Z_t$ are lower bounded by a positive constant due to the boundedness of $h(\cdot)$ (see \cref{subsection filtering problems}), so $\frac{1}{Z_t}$ is uniformly upper bounded and, therefore, not a concern in the error analysis.
\eqref{eq. bias caused by artificial evolution} tells that the error analysis of a particle filter can be performed in a recursive fashion, where one analyzes the error of the filter at time $t_{i+1}$ after estimating the error at time $t_i$.
Therefore, the key to proving our result lies in investigating the first three terms on the right hand side of this equality. 
We note that the first and the third terms can be easily analyzed using the techniques in the classical literature \cite{del2000branching,crisan2001particle,bain2008fundamentals}.
%and the error caused by model reduction can be analyzed using the tools in \cite{fang2021stochastic,calzolari2006approximation}.
Consequently, the most challenging part is to analyze the second term, which corresponds to the error caused by the artificial evolution step. 
}

\textcolor{blue}{Technically, we estimate the fourth order moment of the error caused by artificial evolution.	
Notice that for any function $\phi$ satisfying \eqref{eq. sensitivity condition of phi}, we can find a positive constant $\tilde C_{\phi}$ such that
 \begin{align} \label{eq. tilde hat convergence}
\mathbb E\left[ \left| \tilde \pi_{M,t_{i}}(\phi) - \hat \pi_{M,t_{i}}(\phi)\right|^4 \right]
&= \mathbb E\left[ \frac{1}{M^4}\left| \sum_{j=1}^M \phi(\hat \kappa_j(t_i), \bar x_j(t_i)) - \phi(\bar \kappa_j(t_i), \bar x_j(t_i))\right|^4 \right] \\
&\leq \frac{C^4_{\phi} }{M^4} \sum_{j=1}^{M} \mathbb E\left[\|\bar \kappa_{j}(t_{i}) - \hat \kappa_{j}(t_{i}) \|^4_2 \left(1+\|\bar x_{j}(t_{i})\|^q_2\right)^4\right] \notag\\
&\leq \frac{\tilde C_{\phi}}{M^2}\mathbb E\left[ \left(1+\|\bar x_{j}(t_{i})\|^q_2\right)^4\right] \notag
\end{align}
where the second line follows from the midpoint theorem, and the last line follows from \Cref{cond. conditions on the artificial noise 1}.
Therefore, we can analyze the effect of artificial evolution by checking whether $K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi$ satisfies \eqref{eq. sensitivity condition of phi} and estimating $\mathbb E\left[ \left(1+\|\bar x_{j}(t_{i})\|^q_2\right)^4\right]$, the former of which corresponds to the parameter sensitivity analysis of the transition kernel. 
}

\textcolor{blue}{Following this idea, in \Cref{subsection proof parameters}, we use the parameter sensitivity analysis to show that the second term on the right hand side of \eqref{eq. bias caused by artificial evolution} is of order $\frac{1}{\sqrt{M}}$.
Specifically, we first prove in \Cref{subsection proof parameters} that both the state vector and the parameter sensitivity for the transition kernel grow mildly under the assumed conditions (\cref{proposition finiteness of moments} and \cref{proposition Kphi}). 
Then, based on these results and \eqref{eq. tilde hat convergence}, we can find a constant $\hat C_{y}$ for any $y\in\mathbb R^{m}$ such that
	\begin{align*}
	\mathbb E\left[ 
		\big| \text{the second term on the RHS of }\eqref{eq. bias caused by artificial evolution} \big|^4 \Big| Y(t_{i+1})=y  \right]  
	%&\leq 8 \mathbb E\left[ \left|\bar \pi_{M,t_{i},C_{\eta}} (\phi) -\bar \pi_{M,t_{i-1},C_{\eta}} (K_{t_{i}-t_{i-1}}\ell_{y_{i}} \phi)  \right|^4 \left| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right. \right]   \\
	%&\quad +8\mathbb E\left[ \left|\bar \pi_{M,t_{i-1},C_{\eta}} (K_{t_{i}-t_{i-1}}\ell_{y_{i}} \phi) -\bar \pi_{M,t_{i-1},0} (K_{t_{i}-t_{i-1}}\ell_{y_{i}} \phi) \right|^4 \left| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right. \right]  \\
	\leq \frac{\hat C_{y}}{M^2},
	\end{align*}
	which indicates that the error caused by artificial evolution is of order $\frac{1}{\sqrt{M}}$ (see \Cref{remark bias}).
	Finally, based on the obtained results, we prove the convergence of the established RPF  by mathematical induction in \Cref{subsection proof main result}.
}

\subsection{Parameter sensitivities for transition kernels and the analysis of the error introduced by artificial evolution} \label{subsection proof parameters}
\textcolor{blue}{In this subsection, we use the parameter sensitivity analysis to estimate the error introduced by the artificial evolution and show that it vanishes as the particle population goes to infinity. 
Recall that the key is to show  $K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi$ satisfying \eqref{eq. sensitivity condition of phi} and moments of particles being bounded from above (see \eqref{eq. tilde hat convergence}).
}

First, \Cref{assumption for full model} and \Cref{assumption non-negativity of tau-leaping algorithm} suggest that any moment of the state vector is bounded, and, therefore, the moments of particles are also bounded.

\begin{proposition}[Adapted from {\cite[Lemma 5.1]{gupta2013unbiased}} and {\cite[Theorem 4.5]{rathinam2016convergence}}]\label{proposition finiteness of moments}
	If \Cref{assumption for full model} holds, then for all $p>0$, there exists a positive constant $C_p$ such that 
	\begin{align*}
	\mathbb E\left[ \left. \left\|X^{N,\gamma_1}(t)\right\|^{p}_2 ~\right| \mathcal K= \kappa, X^{N,\gamma_1}(0)=x \right] &\leq 
	\left( \left\|x\right\|^{p}_2
	+ C_p t \right) \text{e}^{C_p t}\\
	\mathbb E\left[ \left. \left\|X^{\gamma_1}(t)\right\|^{p}_2 ~\right| \mathcal K = \kappa, X^{\gamma_1}(0)=x \right] &\leq 
	\left( \left\|x\right\|^{p}_2
	+ C_p t \right) \text{e}^{C_p t}
	\end{align*}
	for any $t>0$ and $(\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$.
	If moreover \Cref{assumption non-negativity of tau-leaping algorithm} holds, then for $p>0$, there exists a constant $C_{p,\tau}$ such that 
	\begin{align*}
	\sup_{t\in[0,T]} 
	\mathbb E \left[ \left. \left\| X^{N,\gamma_1}_{\tau}(t) \right\|_2^p \right|  \mathcal K=\kappa, X^{N,\gamma_1}_{\tau}(t)=x  \right]
	\leq 	\left( \left\|x\right\|^{p}_2
	+ 1\right) \text{e}^{C_{p,\tau} t }
	\end{align*} 
	for all $(\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$.
\end{proposition}
\begin{proof}
	The results for the full model and the PDMP are adapted from {\cite[Lemma 5.1]{gupta2013unbiased}}; the result for the tau-leaping method is adapted from {\cite[Theorem 4.5]{rathinam2016convergence}}.
\end{proof}

Then, we look at the parameter sensitivity for the CTMC, tau-leaping model, and PDMP. 
Given an initial condition $(\kappa,x)$ and a time point $t$, we term
\begin{align*}
	\Psi^{N}_{t,g}(\kappa,x) &= \mathbb E \left[ g\left(X^{N,\gamma_1}(t)\right) \left|~\mathcal K\triangleq \kappa,  X^{N,\gamma_1}(0)=x\right.\right],  \\
	\Psi^{N,\tau}_{t,g}(\kappa,x) &= \mathbb E \left[ g\left(X^{N,\gamma_1}_{\tau}(t)\right) \left|~\mathcal K\triangleq \kappa,  X^{N}(0)=x\right.\right], \\
	\Psi_{t,g}(\kappa,x) &= \mathbb E \left[ g\left(X^{\gamma_1}(t)\right) \left|~\mathcal K\triangleq \kappa,  X^{N,\gamma_1}(0)=x\right.\right]  
\end{align*}
as the conditional expectations of function $g$ for the CTMC, tau-leaping model, and PDMP, respectively.
Then, the parameter sensitivity for these models are defined, respectively, by $\frac{\partial \Psi^N_{t,g}(\kappa,x) }{\partial \kappa}$, $\frac{\partial \Psi^{N,\tau}_{t,g}(\kappa,x) }{\partial \kappa}$, and $\frac{\partial \Psi_{t,g}(\kappa,x) }{\partial \kappa}$.
The literature \cite{gupta2018estimation} shows that the parameter sensitivity for the full model can be computed by 
\begin{small}
\begin{align}
&\frac{\partial \Psi^N_{t,g}(\kappa,x) }{\partial \kappa} \label{eq. parameter sensitivity for SCRNs} \\
&= \sum_{j=1}^{r} \mathbb{E}
\left[
\left. 
\int_{0}^{t} \frac{\partial \lambda^{N}_{j}\left(\kappa, X^{N,\gamma_1}(s)\right)}{\partial \kappa} 
\Delta^N_j \Psi^N_{t-s,g}\left(\kappa,X^{N,\gamma_1}(s)\right) 
\dd s
\right| ~\mathcal K=\kappa,  X^{N}(0)=x 
\right] \notag
\end{align}
\end{small}where $\Delta^N_j \Psi^N_{t-s,g}\left(\kappa,x\right)\triangleq \Psi^N_{t-s,g}\left(\kappa,x+\Lambda^N \zeta_j\right)- \Psi^N_{t-s,g}\left(\kappa,x\right)$.
Similarly, by mathematical induction, we can show that the parameter sensitivity for the tau-leaping model (with a deterministic time-discretization scheme) can be computed by 
\begin{small}
\begin{align}
&\frac{\partial \Psi^{N,\tau}_{t,g}(\kappa,x) }{\partial \kappa} \label{eq parameter sensitivity for the tau-leaping method} \\
&= \sum_{j=1}^{r} \mathbb{E}
\Bigg[
\sum_{\tau_i<t}  (\tau_{i+1}\wedge t -\tau_i)\frac{\partial \lambda^{N}_{j}\left(\kappa, X^{N,\gamma_1}_\tau (\tau_i)\right)}{\partial \kappa} 
\Delta^N_j \Psi^N_{t-s,g}\left(\kappa,X^{N,\gamma_1}_{\tau}(\tau_{i+1})\right) \notag \\
& \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad
\bigg| ~\mathcal K=\kappa,  X^{N,\gamma_1}_{\tau}(0)=x 
\bigg]. \notag
\end{align}
\end{small}\textcolor{blue}{(Note that $\frac{\partial \Psi^{N,\tau}_{t,g}(\kappa,x) }{\partial \kappa}$ computes the parameter sensitivity when the tau-leaping model is viewed as the ground truth. It is not necessarily equal or even close to $\frac{\partial \Psi^N_{t,g}(\kappa,x) }{\partial \kappa}$, the parameter sensitivity for the full model.)}
%where $	\Psi^{N,\tau}_{t,g}(\kappa,x) = \mathbb E \left[ g\left(X^{N,\gamma_1}_{\tau}(t)\right) \left|~\mathcal K\triangleq \kappa,  X^{N}(0)=x\right.\right]. $
Finally, the literature \cite{gupta2019sensitivity} tells that under \Cref{assumption convergence of the initial condition}, \Cref{assumption for full model}, and \Cref{assumption for PDMPs}, the parameter sensitivity for the PDMP satisfies
\begin{equation}\label{eq. parameter sensitivity PDMP}
	\frac{\partial \Psi_{t,g}(\kappa,x) }{\partial \kappa} = \lim_{N\to\infty} \frac{\partial \Psi^N_{t,g}(\kappa,x) }{\partial \kappa}
\end{equation}
if $g$ is bounded, continuously differentiable.
Using these results, we can further prove that the parameter sensitivity for the transition kernel is at most polynomially growing with respect to the state argument (see \Cref{proposition Kphi}).

\begin{proposition}(Polynomially growing rate of the parameter sensitivity for the transition kernel)\label{proposition Kphi}
	For any measurable function $\phi$, we denote 
	\begin{align*}
		\left(K^{N,\gamma_1}_t \phi \right)(\kappa, x) &\triangleq \mathbb E_{\mathbb P} \left[ \phi\left(\mathcal K, X^{N,\gamma_1}(t)\right) \left|~\mathcal K=\kappa,  X^{N}(0)=x\right.\right], \\
		\left(K^{N,\gamma_1,\tau}_t \phi \right)(\kappa, x) &\triangleq \mathbb E_{\mathbb P} \left[ \phi\left(\mathcal K, X^{N,\gamma_1}_{\tau}(t)\right) \left|~\mathcal K=\kappa,  X^{N}(0)=x\right.\right], \\
		\left(K^{\gamma_1}_t \phi \right)(\kappa, x) &\triangleq \mathbb E_{\mathbb P} \left[ \phi\left(\mathcal K, X^{\gamma_1}(t)\right) \left|~\mathcal K=\kappa,  X^{\gamma_1}(0)=x\right.\right].
	\end{align*}
	If $\phi:\Theta\times \mathbb R^{n}_{\geq 0} \to \mathbb R$ 
	satisfies the requirement in \cref{thm main}, then the following results hold.
	\begin{itemize}
		\item If \Cref{assumption for full model} holds, then for any $t>0$ there exists a constant $C_{t,\phi}$ such that $\left\| \frac{ \partial \left(K^{N,\gamma_1}_t \phi \right)(\kappa, x) }{\partial \kappa}\right\|_{2} 
		\leq C_{t,\phi} \left(1+ \|x\|^q_2\right)$ for all $ (\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$.
		\item If \Cref{assumption non-negativity of tau-leaping algorithm} and \Cref{assumption for full model} hold, then for any $t>0$ there exists a constant $C_{t,\phi,\tau}$ such that $\left\| \frac{ \partial \left(K^{N,\gamma_1,\tau}_t \phi \right)(\kappa, x) }{\partial \kappa}\right\|_{2} 
		\leq C_{t,\phi,\tau} \left(1+ \|x\|^q_2\right)$ for all $ (\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$.
		\item If \Cref{assumption convergence of the initial condition}, \Cref{assumption for full model}, and \Cref{assumption for PDMPs} hold, then for any $t>0$ and $ (\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$ there holds  $	\left\| \frac{ \partial \left(K^{\gamma_1}_t \phi \right)(\kappa, x) }{\partial \kappa}\right\|_{2} \leq C_{t,\phi} \left(1+ \|x\|^q_2\right)$,
		where $C_{t,\phi}$ is the same as that in the first result.
	\end{itemize}
\end{proposition}

\begin{proof}
    We first prove the result for the transition kernel of the full model.
    By definition, we can write the derivative of the transition kernel by 
    \begin{align}
    \frac{ \partial K^{N,\gamma_1}_t \phi (\kappa, x) }{\partial \kappa} \notag
    =& \mathbb E \left[ \left. \frac{\partial \phi\left(\kappa, X^{N,\gamma_1}(t)\right)}{\partial \kappa} \right|~\mathcal K=\kappa,  X^{\gamma_1}(0)=x \right]
    +
    \left.\frac{\partial \Psi^{N}_{t,\phi(\kappa, \cdot)}(\theta,x) }{\partial \theta}\right|_{\theta=\kappa}. 
    \end{align}
    %the first term follows from the dominant convergence theorem.
    By \cref{eq. sensitivity condition of phi} and \cref{proposition finiteness of moments}, we can find a positive constant $C^1_{t,\phi}$ such that 
    \begin{equation}\label{eq. sensitivity analysis help 1}
    \mathbb E \left[ \left. \left\| \frac{\partial \phi\left(\kappa, X^{N,\gamma_1}(t)\right)}{\partial \kappa}\right\|_2 \right|~\mathcal K=\kappa,  X^{\gamma_1}(0)=x \right]
    \leq C^1_{t,\phi}\left( 1
    + \|x\|^q_2 \right)
    \end{equation}
    for all $(\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$.
    Also, by \eqref{eq. parameter sensitivity for SCRNs} and the boundedness of $\phi$, there holds
    \begin{align}
    \left\| \left.\frac{\partial \Psi^{N}_{t,\phi(\kappa, \cdot)}(\theta,x) }{\partial \theta}\right|_{\theta=\kappa}  \right\|_2
    &\leq  2\|\phi\|_{\infty}\sum_{j=1}^{r} \left\|\mathbb{E}
    \left[
    \left. 
    \int_{0}^{t} \frac{\partial \lambda^{N}_{j}\left(\kappa, X^{N,\gamma_1}(s)\right)}{\partial \kappa} 
    \dd s
    \right| ~\mathcal K=\kappa,  X^{N}(0)=x 
    \right]\right\|_2 \notag \\
    & \leq  2\|\phi\|_{\infty}\sum_{j=1}^{r} \mathbb{E}
    \left[
    \left. 
    \int_{0}^{t} \left\| \frac{\partial \lambda^{N}_{j}\left(\kappa, X^{N,\gamma_1}(s)\right)}{\partial \kappa} \right\|_2
    \dd s
    \right| ~\mathcal K=\kappa,  X^{N}(0)=x 
    \right] \notag 
    \end{align}
    where the second inequality follows from Jensen's inequality and the triangle inequality.
    Therefore by \Cref{proposition finiteness of moments} and \Cref{assumption for full model}, we can find a constant $C^2_{t,\phi}$ such that 
    \begin{equation}\label{eq. sensitivity analysis help 2}
    \left\| \left.\frac{\partial \Psi^{N}_{t,\phi(\kappa, \cdot)}(\theta,x) }{\partial \theta}\right|_{\theta=\kappa}\right\|_2
    \leq  C^2_{t,\phi}\left( 1
    + \|x\|^q_2 \right)
    \qquad \forall (\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}.
    \end{equation}
    Finally, by combing \eqref{eq. sensitivity analysis help 1} and \eqref{eq. sensitivity analysis help 2}, we prove the result for the transition kernel of the full model (the first result).
    
    By the same argument, we can also prove the second result. 
    %For the third result, we need to use an additional result from \cite{gupta2019sensitivity}:
    %if \Cref{assumption convergence of the initial condition}, \Cref{assumption for full model}, and \Cref{assumption for PDMPs} hold, then for any $t>0$, $ (\kappa,x) \in \Theta\times \mathbb R^{n}_{\geq 0}$ and bounded, continuously differentiable function $g$, there holds
    %$\lim_{N\to\infty} \frac{\partial  }{\partial \kappa} \Psi^{N}_{t,g}(\kappa,x)=  \frac{\partial }{\partial \kappa}\Psi_{t,g}(\kappa,x) $, where $\Psi_{t,g}(\kappa,x)  = \mathbb E_{\mathbb P} \left[ g\left( X^{\gamma_1}(t)\right) \left|~\mathcal K=\kappa,  X^{\gamma_1}(0)=x\right.\right]$. 
    For the third result, we can learn from \eqref{eq. parameter sensitivity PDMP} that $\Psi_{t,\phi(\kappa, \cdot)}(\theta,x)$ satisfies \eqref{eq. sensitivity analysis help 2}.
    Moreover, by \cref{eq. sensitivity condition of phi} and \cref{proposition finiteness of moments}, we can show that the quantity $\phi\left(\kappa, X^{\gamma_1}(t)\right)$ also satisfies \eqref{eq. sensitivity analysis help 1}.
    Therefore, the third result is proven. 
\end{proof}


\begin{remark}[Analysis of the error introduced by artificial evolution]{\label{remark bias}}
	\textcolor{blue}{
	Now, we use the obtained propositions to show that the second term on the right hand side of \eqref{eq. bias caused by artificial evolution} is of the order $1/\sqrt{M}$.}
	%Recall that for a given RPF, we briefly denote  $K_t$ as the transition kernel applied in the filter, $\hat \pi_{M,t_i}(\phi)$ as the estimate of function $\phi$ based on the resampled particles, and $\tilde  \pi_{M,t_i}(\phi)$ as the estimate of $\phi$ based on the noise-perturbed particles (see \eqref{eq. notations}).}
%	By the midpoint theorem, we can show that for any $\phi$ satisfying the requirement in \Cref{thm main}, there exists a constant ${C_{\phi}}$ such that
%    \begin{equation*}
%      \tilde \pi_{M,t_{i}}(\phi) - \hat \pi_{M,t_{i}}(\phi)
%     = \frac{C_{\phi}}{M}\sum_{j=1}^{M} \left\|\bar \kappa_{j}(t_{i}) - \hat \kappa_{j}(t_{i})  \right\|_{2}
%      \left(1+\|\bar x_{j}(t_{i})\|^q_2\right).
%     \end{equation*}
%     Note that $(\sum_{j=1}^M a_j)^4=(\sum_{j=1}^M  a_j)^2(\sum_{j=1}^M  a_j)^2\leq M^2 (\sum_{j=1}^M  a^2_j)^2 \leq M^3 \sum_{j=1}^M  a^4_i$ for any series $\{a_j\}$.
%     Then, we can find another positive constant $\tilde C_{\phi}$ such that
%     	\begin{align} %\label{eq. tilde hat convergence}
%     \mathbb E\left[ \left| \tilde \pi_{M,t_{i}}(\phi) - \hat \pi_{M,t_{i}}(\phi)\right|^4 \right]
%     &\leq \frac{C^4_{\phi} }{M} \sum_{j=1}^{M} \mathbb E\left[\|\bar \kappa_{j}(t_{i}) - \hat \kappa_{j}(t_{i}) \|^4_2 \left(1+\|\bar x_{j}(t_{i})\|^q_2\right)^4\right] \notag\\
%     &\leq \frac{\tilde C_{\phi}}{M^2}
%     \end{align}
%     where the last line follows from \Cref{cond. conditions on the artificial noise 1} and \Cref{proposition finiteness of moments}.}
    \textcolor{blue}{
    Note that if $\phi$ satisfies the requirement in  \Cref{thm main}, the function $\ell_{y} \phi$ (for any $y\in\mathbb R^{m}$) also satisfies this requirement, because the likelihood function $\ell_{y}$ is bounded and has no dependence on the argument $\kappa$.
    Consequently, by \cref{proposition Kphi}, the function $K_{\Delta t_i} \ell _{Y(t_{i+1})}\phi$ also satisfies the requirement in  \Cref{thm main} under the proposed conditions.
    Moreover, we can conclude by \cref{proposition finiteness of moments} that any moment of particles is bounded from above.
    Finally, applying these results to \eqref{eq. tilde hat convergence}, we can find a positive constant $\hat C_{y}$ such that 
     \begin{align*}
    \mathbb E\left[ 
    \big| \text{the second term on the right hand side of }\eqref{eq. bias caused by artificial evolution} \big|^4 \left| Y^{N,\gamma_1}(t_{i+1})=y \right. \right]  
    %&\leq 8 \mathbb E\left[ \left|\bar \pi_{M,t_{i},C_{\eta}} (\phi) -\bar \pi_{M,t_{i-1},C_{\eta}} (K_{t_{i}-t_{i-1}}\ell_{y_{i}} \phi)  \right|^4 \left| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right. \right]   \\
    %&\quad +8\mathbb E\left[ \left|\bar \pi_{M,t_{i-1},C_{\eta}} (K_{t_{i}-t_{i-1}}\ell_{y_{i}} \phi) -\bar \pi_{M,t_{i-1},0} (K_{t_{i}-t_{i-1}}\ell_{y_{i}} \phi) \right|^4 \left| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right. \right]  \\
    \leq \frac{\hat C_{y}}{M^2},
    \end{align*}
    which suggests that the bias contributed by artificial evolution is of order $\frac{1}{\sqrt{M}}$.
   }
    
%    {
%    \cref{proposition finiteness of moments} suggests that any moment of particles is bounded from above.
%    Note that if $\phi$ satisfies the requirement in  \Cref{thm main}, the function $\ell_{y} \phi$ (for any $y\in\mathbb R^{m}$) also satisfies this requirement, as $\ell_{y}$ is bounded and has no dependence on the argument $\kappa$.
%    By the technique of \cite[equation (2.10)]{crisan2001particle}, we can conclude 
%    \begin{align*}
%    	&\big| \text{the second term on the right hand side of }\eqref{eq. bias caused by artificial evolution}\big| \\
%    	&\leq 
 %   	\frac{\|\phi\|_{\infty}\left| \tilde \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})})-\hat \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})})\right|}
 %   	{\tilde \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})})} \\
 %   	&\quad+    	\frac{\left| \tilde \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})}\phi)-\hat \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})}\phi)\right|}
 %   	{\tilde \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})})}.
%    \end{align*}
%    In this formula, the term $1/\tilde \pi_{M,t_{i}} ( K_{t_{i+1}-t_{i}} \ell _{Y^{N,\gamma_1}(t_{i+1})})$ is bounded from above due to the boundedness of $h$ (see the definition of the likelihood function low \eqref{eq. recurssive expression 2}).
%    Also, notice that if $\phi$ satisfies the requirement in  \Cref{thm main}, the function $\ell_{y} \phi$ (for any $y\in\mathbb R^{m}$) also satisfies this requirement, as $\ell_{y}$ is bounded and has no dependence on the argument $\kappa$.
%     Thus, applying all these facts, \Cref{proposition Kphi}, and \eqref{eq. tilde hat convergence} to the above formula, we can conclude 
%    }
\end{remark}


\subsection{Proving the main result by mathematical induction} {\label{subsection proof main result}}

\textcolor{blue}{In this subsection, we prove \cref{thm main} using the result obtained in the previous section.}

\textcolor{blue}{Before proving the main result, we first analyze the error caused by model reduction and show that it vanishes as the reduced model approaches the full model. 
}
Here, we define observations for the tau-leaping algorithm and the PDMP by
\begin{align*}
Y^{N,\gamma_1,\tau}(t_i)&= h\left(X^{N,\gamma_1}_{\tau}(t_i)\right)  + W(t_i) \qquad && \forall i\in \mathbb N_{>0}, \\
Y^{\gamma_1}(t_i)&= h\left(X^{\gamma_1}_{\tau}(t_i)\right)  + W(t_i) \qquad && \forall i\in \mathbb N_{>0},
\end{align*} 
and term $\mathcal Y^{N,\gamma_1,\tau}_{t_i}$ and $\mathcal Y^{\gamma_1}_{t_i}$ as the $\sigma$-algebras generated, respectively, by $Y^{N,\gamma_1,\tau}(\cdot)$ and $Y^{\gamma_1}(\cdot)$ up to the time $t_i$.
Note that for any bounded measurable function $\phi$, the conditional expectations $\mathbb E \left[ \phi \left( \mathcal K, X^{N,\gamma_1}(t_i) \right) \big| \mathcal Y^{N,\gamma_1}_{t_i} \right]$, $\mathbb E \left[ \phi \left( \mathcal K, X^{N,\gamma_1}_{\tau}(t_i) \right) \big| \mathcal Y^{N,\gamma_1,\tau}_{t_i} \right]$, and $\mathbb E \left[ \phi \left( \mathcal K, X^{\gamma_1}(t_i) \right) \big| \mathcal Y^{\gamma_1}_{t_i} \right]$, are respectively $\mathcal Y^{N,\gamma_1}_{t_i}$-measurable, $\mathcal Y^{N,\gamma_1,\tau}_{t_i}$-measurable, and $\mathcal Y^{\gamma_1}_{t_i}$-measurable.
So, there exist measurable functions $\hat f^{N,\gamma_1}_{\phi,t_i}$, $\hat f^{N,\gamma_1,\tau}_{\phi,t_i}$, and $\hat f^{\gamma_1}_{\phi,t_i}$, such that 
\begin{align*}
    \hat f^{N,\gamma_1}_{\phi,t_i}\left( Y^{N,\gamma_1}_{1:i}\right) &= \mathbb E_{\mathbb P} \left[ \phi \left( \mathcal K, X^{N,\gamma_1}(t_i) \right) \big| \mathcal Y^{N,\gamma_1}_{t_i} \right] \\
	\hat f^{N,\gamma_1,\tau}_{\phi,t_i}\left( Y^{N,\gamma_1,\tau}_{1:i}\right) &= \mathbb E_{\mathbb P} \left[ \phi \left( \mathcal K, X^{N,\gamma_1}_{\tau}(t_i) \right) \big| \mathcal Y^{N,\gamma_1,\tau}_{t_i} \right] \\
	\hat f^{\gamma_1}_{\phi,t_i}\left( Y^{\gamma_1}_{1:i}\right) &= \mathbb E_{\mathbb P} \left[ \phi \left( \mathcal K, X^{\gamma_1}(t_i) \right) \big| \mathcal Y^{\gamma_1}_{t_i} \right]
\end{align*}
where $Y^{N,\gamma_1}_{1:i}\triangleq \left(Y^{N,\gamma_1}(t_1),\dots, Y^{N,\gamma_1}(t_i)\right)$, $Y^{N,\gamma_1,\tau}_{1:i}\triangleq \left(Y^{N,\gamma_1,\tau}(t_1),\dots, Y^{N,\gamma_1,\tau}(t_i)\right)$, and $Y^{\gamma_1}_{1:i}\triangleq \left(Y^{\gamma_1}(t_1),\dots, Y^{\gamma_1}(t_i)\right)$.
Here, $ \hat f^{N,\gamma_1,\tau}_{\phi,t_i}\left( Y^{N,\gamma_1,\tau}_{1:i}\right)$ and $\hat f^{\gamma_1}_{\phi,t_i}\left( Y^{\gamma_1}_{1:i}\right)$ are exact filters for the tau-leaping model and PDMP, respectively.

The following proposition states that $\hat f^{N,\gamma_1,\tau}_{\phi,t_i}\left( Y^{N,\gamma_1}_{1:i}\right) $ and $\hat f^{\gamma_1}_{\phi,t_i}\left( Y^{N,\gamma_1}_{1:i}\right)$ converge in probability to the exact filter $\pi^{N,\gamma_1}_{t_i}(\phi)$ as $|\tau|\to 0$ and $N\to\infty$, respectively.
Therefore, to show the final result, we only need to check that $\bar \pi^{N,\gamma_1}_{M,t_i}(\phi)$, $\bar \pi^{N,\gamma_1,\tau}_{M,t_i}$, and $\bar \pi^{N,\gamma_1, H}_{M,t_i}$ converge respectively to $\hat f^{N,\gamma_1}_{\phi,t_i}\left( Y^{N,\gamma_1}_{1:i}\right)$, $\hat f^{N,\gamma_1,\tau}_{\phi,t_i}\left( Y^{N,\gamma_1}_{1:i}\right)$, and $\hat f^{\gamma_1}_{\phi,t_i}\left( Y^{N,\gamma_1}_{1:i}\right)$ as $M\to\infty$.

\begin{proposition}\label{prop fang}[Adapted from {\cite{fang2021stochastic}}]~
	\begin{itemize}
		\item If \Cref{assumption non-negativity of tau-leaping algorithm}, \Cref{assumption convergence of tau-leaping algorithm}, and \Cref{assumption for full model} hold, then for any $i\in\mathbb N_{>0}$, $N>0$, and bounded continuous function $\phi$, there is the convergence result $\hat f^{N, \gamma_1, \tau}_{\phi,t_i} \left(Y^{N,\gamma_1}_{1:i}\right) \stackrel{\mathbb P}{\to} \pi^{N,\gamma_1}_{t_i}(\phi)$ as $|\tau|\to0$.
		\item If \Cref{assumption convergence of the initial condition} and \Cref{assumption for full model} hold, then there is the convergence result $\lim_{N\to\infty}\mathbb P \left( \left|\hat f^{\gamma_1}_{\phi,t_i} \left(Y^{N,\gamma_1}_{1:i}\right) - \pi^{N,\gamma_1}_{t_i}(\phi)\right| >\delta\right)=0$
		 for any $i\in\mathbb N_{>0}$, $\delta>0$ and bounded continuous function $\phi$.
	\end{itemize}
\end{proposition}

\begin{proof}
	The second result has been proven in \cite{fang2021stochastic}; following the technique in \cite{fang2021stochastic}, one can easily prove the first result.
	Here, we give the outline of the proof. 
	
	Let's define Girsanov random variables $Z^{N,\gamma_1}(t_i)\triangleq \prod_{j=1}^i g\left(X^{N,\gamma_1}(t_j), Y^{N,\gamma_1}(t_j)\right)$ and $Z^{N,\gamma_1,\tau}(t_i)\triangleq \prod_{j=1}^i g\left(X^{N,\gamma_1}_{\tau}(t_j), Y^{N,\gamma_1,\tau}(t_j)\right)$ for the full dynamical model and the tau-leaping algorithm, respectively, where $g(x,y)=\exp\left(\sum_{\ell=1}^m h_{\ell}(x)y_{\ell}-h^2_{\ell}(x)/2\right)$.
	Since the reciprocals of $Z^{N,\gamma_1}(t_i)$ and $Z^{N,\gamma_1,\tau}(t_i)$ are both martingales, we can then define reference probability $\mathbb P^{N,\gamma_1}$ and $\mathbb P^{N,\gamma_1,\tau}$ by 
	\begin{equation*}
	\left.\frac{\dd \mathbb P^{N,\gamma_1}}{\dd \mathbb P}\right|_{\mathcal F_{t_i}} = \left(Z^{N,\gamma_1}(t_i)\right)^{-1} 
	\qquad
	\text{and}
	\qquad
	\left.\frac{\dd \mathbb P^{N,\gamma_1,\tau}}{\dd \mathbb P}\right|_{\mathcal F_{t_i}} = \left(Z^{N,\gamma_1,\tau}(t_i)\right)^{-1}. 
	\end{equation*}
	In the reference probability, the process and the observation are independent, and the observations become a sequence of independent $m$-variate standard Gaussian variables.
	
	According to \cite[Theorem 2.6]{calzolari2006approximation}, the first result holds if for any $i>0$, we can construct random processes $\tilde X^{N,\gamma_1}(\cdot)$, $\tilde X^{N,\gamma_1,\tau}(\cdot)$, $\tilde Y (\cdot)$,  $\tilde Z^{N,\gamma_1}(\cdot)$, and $Z^{N,\gamma_1,\tau}(\cdot)$ on a common probability space $\left(\tilde \Omega, \tilde {\mathcal F},  \mathbb Q \right)$ such that the following conditions hold.
	\begin{enumerate} [label=a.\arabic*]
		\item Random variables $\left( \tilde X^{N,\gamma_1}(\cdot), \tilde Y (\cdot), \tilde Z^{N,\gamma_1}(t_i)  \right) \in \mathbb D_{\mathbb R^{n}}[0,t_i] \times \mathbb R^{m\times i} \times \mathbb R$ have the same law as  $\left( X^{N,\gamma_1}(\cdot), Y^{N,\gamma_1}(\cdot), Z^{N,\gamma_1}(t_i)  \right)$ on $\left(\Omega,\mathcal F, \mathbb P^{N,\gamma_1} \right)$. \label{a.1}
		\item Random variables $\left( \tilde X^{N,\gamma_1,\tau}(\cdot), \tilde Y (\cdot), \tilde Z^{N,\gamma_1,\tau}(t_i)  \right) \in \mathbb D_{\mathbb R^{n}}[0,t_i] \times \mathbb R^{m\times i} \times \mathbb R$ have the same law as  $\left( X^{N,\gamma_1}_{\tau}(\cdot), Y^{N,\gamma_1,\tau}(\cdot), Z^{N,\gamma_1,\tau}(t_i)  \right)$ on $\left(\Omega,\mathcal F, \mathbb P^{N,\gamma_1,\tau} \right)$. \label{a.2}
		\item $\hat f^{N,\gamma_1,\tau}_{\phi,t_i} \left(\tilde Y_{1:i}\right) \stackrel{\mathbb P}{\to} \hat f^{N,\gamma_1}_{\phi,t_i} \left(\tilde Y_{1:i}\right) $ as $|\tau|\to0$, where $\tilde Y_{1:i}=\left(\tilde Y(t_1),\dots, \tilde Y(t_i)\right)$. \label{a.3}
		\item $\lim_{|\tau|\to\infty} \mathbb E_{\mathbb Q} \left[ \left|  \tilde Z^{N,\gamma_1}(t_i) - \tilde Z^{N,\gamma_1,\tau}(t_i) \right|\right]=0$. \label{a.4}
	\end{enumerate} 
	
	These random variables and the common probability space can be constructed as follows.
	By the Skorokhod representation theorem and \Cref{assumption convergence of tau-leaping algorithm}, we can find a common probability space $\left( \tilde \Omega_1, \tilde {\mathcal F}_1, \mathbb Q_1 \right)$, on which are defined $\mathbb D_{\mathbb R^{n}}[0,t_i]$-valued variables $\tilde X^{N,\gamma_1}(\cdot)$ and $\tilde X^{N,\gamma_1,\tau}(\cdot)$ that have the same law as $X^{N,\gamma_1}(\cdot)$ and $X^{N,\gamma_1}_{\tau}(\cdot)$ respectively and, moreover, satisfy $\lim_{|\tau|\to\infty}\tilde X^{N,\gamma_1}_\tau(\cdot) = X^{N,\gamma_1}(\cdot)$ $\mathbb Q$-almost surely.
	Let us term $\left\{ \tilde Y (t_j) \right\}_{1\leq j \leq i}$ as a sequence of independent $m$-variate standard Gaussian random variables and $\left( \tilde \Omega_2, \tilde {\mathcal F}_2, \mathbb Q_2 \right)$ as the probability space on which they are defined.
	Finally, the probability space $\left(\tilde \Omega, \tilde {\mathcal F},  \mathbb Q \right)$ is defined by the product of $\left( \tilde \Omega_1, \tilde {\mathcal F}_1, \mathbb Q_1 \right)$ and $\left( \tilde \Omega_2, \tilde {\mathcal F}_2, \mathbb Q_2 \right)$, and the Girsanov random variables are defined by $\tilde Z^{N,\gamma_1}(t_i)\triangleq \prod_{j=1}^i g\left(\tilde X^{N,\gamma_1}(t_j), \tilde Y(t_j)\right)$ and $\tilde Z^{N,\gamma_1,\tau}(t_i)\triangleq \prod_{j=1}^i g\left(\tilde X^{N,\gamma_1,\tau}(t_j), \tilde Y(t_j)\right)$. 
	
	Obviously, such random variables satisfy \ref{a.1} and \ref{a.2}. Moreover, \ref{a.4} follows immediately from the almost sure convergence of  $\tilde X^{N,\gamma_1,\tau}(\cdot)$ to $\tilde X^{N,\gamma_1}(\cdot)$. Finally, \ref{a.3} can be proven by the Kallianpur-Striebel formula together with the aforementioned convergence result.
\end{proof}

Finally, we prove the main theorem using mathematical induction.

\begin{proof}[The Proof of \cref{thm main}]
    Here, we prove the result using the simplified notations in \eqref{eq. notations}. 
    Moreover, for a given RPF, we briefly denote the associated measurable function ($\hat f^{N,\gamma_1}_{\phi,t_i}$, $\hat f^{N,\gamma_1,\tau}_{\phi,t_i}$, or $\hat f^{\gamma_1}_{\phi,t_i}$) by $\hat f_{\phi,t_i}$.
    For $t_0$, we term $\hat f_{\phi, t_0} (Y^{N,\gamma_1}_{1:0})$ as the expectation of $\phi$ with respect to the initial distribution. %and $\tilde \pi_{M,t_0}(\phi) \triangleq \frac{1}{M} {\sum_{j=1}^{M} \phi(\bar \kappa_j(t_0), \bar x_j(t_0))}$ as the estimate of $\phi$ based on initial particles.
	
	\Cref{prop fang} tells that to prove the result, we only need to show $\bar \pi_{M,t_i}(\phi) \to \hat f_{\phi, t_i} (Y^{N,\gamma_1}_{1:i})$ in probability as $M\to\infty$.
	In the following, we prove that this convergence actually holds almost surely.
	The proof is in the same spirit as that in the classical literature \cite{crisan2001particle,del2000branching,bain2008fundamentals}, with the difference that we need to additionally consider the moment of particles (see \ref{claim 1}).
	In the sequel, we first make a few claims (see \ref{claim 1}, \ref{claim 2}, and \ref{claim 3} in the following paragraph) and then prove them by mathematical induction.
	Here, proving \ref{claim 2} requires us to look at the finite sampling error (the first term on the right hand side of \eqref{eq. bias caused by artificial evolution}), and proving \ref{claim 3} requires us to analyze the error caused by artificial evolution and resampling (the second and third term on the right hand side of \eqref{eq. bias caused by artificial evolution}).
	Finally, by applying the Borel-Cantelli lemma to \ref{claim 2}, we can show that $\bar \pi_{M,t_i}(\phi) \to \hat f_{\phi, t_i} (Y^{N,\gamma_1}_{1:i})$ almost surely as $M\to\infty$ for any fixed $N$ and $i$, which together with \cref{prop fang} proves the result.
	
	Now, we only need to show  that the following results hold.
		\begin{enumerate}[label=R.\arabic*]
		\item For $i=0$ and any $p>0$, there exists a positive constant $C_{0,p}$ such that the inequality $\mathbb E \left[ \sum_{j=1}^M \frac{\left\| \bar x_j(t_i)\right\|^p_2}{M}\right]\leq C_{0,p}$ holds; for any $i\in\mathbb N_{>0}$, $p>0$, and $y_{1:i}\in\mathbb R^{m\times i}$, there exits a positive constant $C_{i,p,y_{1:i}}$ such that  $$\mathbb E \left[ \left. \sum_{j=1}^M \frac{\left\| \bar x_j(t_i)\right\|^p_2}{M} \right| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right]\leq C_{i,p,y_{1:i}}.$$ \label{claim 1}
		\item  For any $i\in\mathbb N_{>0}$, $y_{1:i}\in\mathbb R^{m\times i}$ and  function $\phi$ satisfying the requirement in \Cref{thm main}, there exists a positive constant $\bar C_{i,\phi,y_{1:i}}$ such that $$\mathbb E \left[ \left. \left| \bar\pi_{M,t_i}(\phi) - \hat f_{\phi, t_i} \left(Y^{N,\gamma_1}_{1:i}\right)\right|^4 \right| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right] \leq\frac{\bar C_{i,\phi,y_{1:i}}}{M^2}.$$ \label{claim 2}
		\item  For $i=0$ and any function $\phi$ satisfying the requirement in \Cref{thm main}, there exists a constant $\tilde C_{0}$  such that $\mathbb E \left[ \left|\tilde \pi_{M,t_0}(\phi) - \hat f_{\phi, t_0} \left(Y^{N,\gamma_1}_{1:i}\right)\right|^4\right] \leq \frac{\tilde C_{0}}{M^2}$;
		for any $i\in\mathbb N_{>0}$, $y_{1:i}\in\mathbb R^{m\times i}$ and function $\phi$ satisfying the requirement in \Cref{thm main}, there exists a positive constant  $\tilde C_{i,\phi,y_{1:i}}$ such that $$\mathbb E \left[ \left. \left| \tilde\pi_{M,t_i}(\phi) - \hat f_{\phi, t_i} \left(Y^{N,\gamma_1}_{1:i}\right)\right|^4 \right| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right] \leq \frac{\tilde C_{i,\phi,y_{1:i}}}{M^2}.$$\label{claim 3}
	\end{enumerate}
	
	For $i=0$, \ref{claim 1} and \ref{claim 3} follow immediately from the third claim of \Cref{assumption for full model} and the fact that initial particles are independently sampled from the initial distribution.
	Then, we prove \ref{claim 1}, \ref{claim 2}, and \ref{claim 3} for a positive integer $i+1$, provide that \ref{claim 1} and \ref{claim 3} hold for the nonnegative integer $i$.
	
	\textit{\ref{claim 1} (for the integer $i+1$):} By \cref{proposition finiteness of moments} and \ref{claim 1} (for the integer $i$), we can find a positive constant $\tilde C_{i+1,p,y_{1:i}}$ for each $p>0$ such that 
	$$\mathbb E \left[ \sum_{j=1}^M \frac{{\left\| x_j(t_{i+1})\right\|^p_2}}{M} \Bigg|  Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1}\right]\leq \tilde C_{i+1,p,y_{1:i}}.$$
	Due to the  boundedness of $h(\cdot)$, the weights $w_j(t_{i+1})$ are uniformly upper bounded by  $\frac{1}{M}\exp\left(2\|h\|_{\infty} \|y_{i+1}\|_1+m\|h\|^2_{\infty}/2\right)$, where $y_{i+1}$ is the last column of $y_{1:i+1}$.
	Therefore, by choosing $C_{i+1,p,y_{1:i}}=\tilde C_{i+1,p,y_{1:i}} \times \exp\left(2\|h\|_{\infty} \|y_{i+1}\|_1+m\|h\|^2_{\infty}/2\right) $, we have the relation $\mathbb E \left[ \sum_{j=1}^M w_j(t_{i+1}){\left\| x_j(t_{i+1})\right\|^p_2} \left|  Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1} \right. \right] \leq C_{i+1,p,y_{1:i}}.$
	Note that the resampling does not change the expectation of the empirical mean, so \ref{claim 1} holds for the integer $i+1$.
	
	\textit{\ref{claim 2} (for the integer $i+1$):}
	According to \ref{claim 3} (for the integer $i$), the key is to analyze the finite sampling error (the first term on right hand side of \eqref{eq. bias caused by artificial evolution}), and we perform the analysis using the technique in \cite{crisan2001particle}. 
	Since we already know $\tilde \pi_{M,t_{i+1}}(\phi)$ converges to $\hat f_{\phi, t_{i+1}}\left(y_{1:i+1}\right)$, we directly compare $\bar\pi_{M,t_{i+1}}(\phi)$ and $\hat f_{\phi, t_{i+1}}\left(y_{1:i+1}\right)$ in this analysis.
	For any function $\phi$ satisfying the requirement in \Cref{thm main},  we define
	\begin{align*}
		\bar \rho_{M,t_i} (\phi)  = {\sum_{j=1}^{M} \phi(\kappa_j, x_j(t_i))} \qquad \forall i\in\mathbb N,
	\end{align*} 
	which is the estimate of the function $\phi$ right before the time point $t_i$.
    For any event  $\left\{\mathcal Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1}\right\}$, this quantity satisfies
	\begin{align}\label{eq. estimate bar rho}
		&\mathbb E \left[ \left. \left| \bar \rho_{M,t_i+1}(\phi) - \tilde f_{(K_{\Delta t_i}\phi), t_i} \left(Y^{N,\gamma_1}_{1:i}\right)\right|^4 \right| Y^{N,\gamma_1}_{1:i}+1=y_{1:i+1} \right] \\
		&\leq 8\mathbb E \left[ \left. \left| \bar \rho_{M,t_i+1}(\phi) - \tilde \pi_{M,t_i}(K_{\Delta t_i} \phi)\right|^4 \right| Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1} \right]  \notag \\
		&\quad+ 8 \mathbb E \left[ \left. \left| \tilde \pi_{M,t_i}(K_{\Delta t_i} \phi) - \tilde f_{(K_{\Delta t_i}\phi), t_i} \left(Y^{N,\gamma_1}_{1:i}\right)\right|^4 \right| Y^{N,\gamma_1}_{1:i}=y_{1:i} \right] \notag \\
		& \leq \frac{3\|\phi\|^4_{\infty}}{M^2}+\frac{\tilde C_{i,(K_{\Delta t_i} \phi),y_{1:i}}}{M^2} \notag
	\end{align}
	where the first inequality follows from $(a+b)^4\leq \left( 2a^2+2b^2\right)^2\leq 8 \left(a^2 +b^2\right)$, and the second inequality follows from the independent increments of particles in the sampling step, \cref{proposition Kphi} (which implies $K_t \phi$ to satisfy \eqref{eq. sensitivity condition of phi}), and \ref{claim 3}.
	%Conditioned on the event  $\left\{\mathcal Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1}\right\}$, there is the relation
	%$\bar\pi_{M,t_{i+1}}(\phi)= {\tilde \pi_{M,t_i}\left(K_{t_{i+1}-t_i} \ell_{y_{i+1}}\phi\right)}/{\tilde \pi_{M,t_i}\left(K_{t_{i+1}-t_i}\ell_{y_{i+1}}\right)},$
	%where $K_t$ is the transition kernel of the process used to construct the RPF, and $\ell_{y_{i+1}}$ is the likelihood function defined in \eqref{eq. recurssive expression 2};
	Moreover, by \cite[(2.10)]{crisan2001particle}, there is
	\begin{align*}
	&\left|\bar\pi_{M,t_{i+1}}(\phi) - \hat f_{\phi, t_{i+1}}\left(y_{1:i+1}\right)\right| \\
	&\leq
	\frac{\left\|\phi\right\|_{\infty}}{\hat f_{ (K_{\Delta t_i}\ell_{y_{i+1}}), t_{i}}\left(y_{1:i}\right)}
	\left|\bar  \rho_{M,t_i+1}\left( \ell_{y_{i+1}}\right)
	 - 
	\hat f_{(K_{\Delta t_i}\ell_{y_{i+1}}), t_{i}}\left(y_{1:i}\right)\right| \\
	& \quad~ +
	\frac{1}{\hat f_{ (K_{\Delta t_i} \ell_{y_{i+1}}), t_{i}}\left(y_{1:i}\right)}
	\left|\bar \rho_{M,t_{i+1}}\left( \ell_{y_{i+1}}\phi\right) 
	- 
	\hat f_{(K_{\Delta t_i} \ell_{y_{i+1}}\phi), t_{i}}\left(y_{1:i}\right)\right|.
	\end{align*}
	Recall that $(a+b)^4\leq 8 \left(a^4+b^4\right)$ for any real $a$ and $b$, and $\hat f_{(K_{\Delta t_i} \ell_{y_{i+1}}), t_i}\left(y_{1:i}\right)$ is lower bounded by a positive constant due to the boundedness of $h(\cdot)$. 
	Therefore, we can find a constant $\bar C_{\ell,\phi,y_{i+1}}$ such that 
	\begin{align*}
	&\left|\bar\pi_{M,t_{i+1}}(\phi) - \hat f_{\phi, t_{i+1}}\left(y_{1:i+1}\right)\right| ^4 \\
	&\leq
	\bar C_{\ell,\phi,y_{i+1}}
	\left|\bar  \rho_{M,t_i+1}\left( \ell_{y_{i+1}}\right)
	- 
	\hat f_{(K_{\Delta t_i} \ell_{y_{i+1}}), t_{i}}\left(y_{1:i}\right)\right|^4 \\
	& \quad~ +\bar C_{\ell,\phi,y_{i+1}}
	\left|\bar \rho_{M,t_{i+1}}\left( \ell_{y_{i+1}}\phi\right) 
	- 
	\hat f_{(K_{\Delta t_i}\ell_{y_{i+1}}\phi), t_{i}}\left(y_{1:i}\right)\right|^4.
	\end{align*}
	conditioned on $\left\{\mathcal Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1}\right\}$.
	%Also, we can conclude that $\ell_{y_{i+1}}$ and $\ell_{y_{i+1}}\phi$ both satisfy \eqref{eq. sensitivity condition of phi}.
	Finally, applying \eqref{eq. estimate bar rho} to this formula, we show 
	\ref{claim 2} for the integer $i+1$.
	
	\textit{\ref{claim 3} (for the integer $i+1$):}
	    According to the result \textit{\ref{claim 2} (for the integer $i+1$)}, in this part,
	    we need to analyze the error caused by artificial evolution and resampling, i.e., the second and third terms on the right hand side of \eqref{eq. bias caused by artificial evolution}.
		If we use the multinomial resampling, then all the resampled particles are independently and identically distributed, and, therefore,  we can conclude % it follows from the independence between resampled particles
	\begin{equation}\label{eq convergence resampling 1}
	\mathbb E \left[ \left. \left| \hat\pi^{N,\gamma_1}_{M,t_{i+1}}(\phi) - \bar \pi^{N,\gamma_1}_{M,t_{i+1}}(\phi)\right|^4 \right| Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1} \right] \leq 
	\frac{\hat C \|\phi\|^4_{\infty}}{M^2}
	\end{equation}
	for a certain constant $\hat C$.
	By  \cite[Exerice 9.1]{bain2008fundamentals} which states that residual resampling introduces the minimum noise among all resampling methods, we can also conclude the above relation for residual resampling. 
	%By \eqref{eq. sensitivity condition of phi}, we can show that 
	%\begin{equation*}
	%\left| \tilde \pi_{M,t_{i+1}}(\phi) - \hat \pi_{M,t_{i+1}}(\phi)\right|
	%\leq \frac{C_{\phi}}{M}\sum_{j=1}^{M} \|\bar \kappa_{j}(t_{i+1}) - \hat \kappa_{j}(t_{i+1})  \|_2 \left(1+\|\bar x_{j}(t_{i+1})\|^q_2\right).
	%\end{equation*}
	%and, therefore,
	%\begin{align*}
	%&\left| \tilde \pi_{M,t_{i+1}}(\phi) - \hat \pi_{M,t_{i+1}}(\phi)\right|^4 
	%\leq \frac{C^4_{\phi} }{M}\sum_{j=1}^{M} \|\bar \kappa_{j}(t_{i+1}) - \hat \kappa_{j}(t_{i+1}) \|^4_2 \left(1+\|\bar x_{j}(t_{i+1})\|^q_2\right)^4
	%\end{align*}
	%where the inequality follows from $(\sum_{j=1}^M a_j)^4=(\sum_{j=1}^M  a_j)^2(\sum_{j=1}^M  a_j)^2\leq M^2 (\sum_{j=1}^M  a^2_j)^2 \leq M^3 \sum_{j=1}^M  a^4_i$.
	%Due to the boundedness of $\Theta$ and \cref{cond. conditions on the artificial noise 1}, we can show that 
	%\begin{equation*}
	%\mathbb E \left[\|\bar \kappa_{j}(t_{i+1}) - \hat \kappa_{j}(t_{i+1})  \|^{4}_2 \bigg| ~\bar x_1(t_{i+1}), \dots, \bar x_{M}(t_{i+1}), Y^{N,\gamma_1}_{1:i+1} \right] \leq \frac{C_{\Theta}}{M^{2}} 
	%\qquad \forall j=1,\dots,M
	%\end{equation*}
	%for some constant $C_{\Theta}$.
	%Combing the above results with \ref{claim 1} (for the integer $i+1$), we can find a positive constant $\hat C_{i,\phi,y_{1:i}}$ such that
	Moreover, by \ref{claim 1} (for the integer $i+1$) and \eqref{eq. tilde hat convergence}, we can also find a positive constant $\hat C_{i,\phi,y_{1:i}}$ such that
	\begin{align}\label{eq convergence resampling 2}
	\mathbb E \left[ \left. \left| \tilde \pi^{N,\gamma_1}_{M,t_{i+1}}(\phi) - \hat \pi^{N,\gamma_1}_{M,t_{i+1}}(\phi)\right|^4 \right| Y^{N,\gamma_1}_{1:i+1}=y_{1:i+1} \right] 
	\leq 
	\frac{\hat C_{i,\phi,y_{1:i}}}{M^2} 
	\end{align}
	Finally, \ref{claim 3} (for the integer $i+1$) follows from \eqref{eq convergence resampling 1} and \eqref{eq convergence resampling 2}.
	%In the above, we have shown \ref{claim 1}, \ref{claim 2}, and \ref{claim 3}; by applying the Borel-Cantelli lemma to \ref{claim 2}, we can show that $\bar \pi_{M,t_i}(\phi) \to \hat f_{\phi, t_i} (Y^{N,\gamma_1}_{1:i})$ almost surely as $M\to\infty$ for any fixed $N$ and $i$, which together with \cref{prop fang} proves the result.
\end{proof}












==> sensitivity_analysis.tex <==
\section{Proof of the main theorem}

In this section, we show the proof of \cref{thm main}.
First, we define an auxiliary process $\left(\tilde {\mathcal K}^{M,\gamma_1}(t), \tilde X^{M,\gamma_1}(t)  \right)$ as follows
\begin{align*}
&\tilde X^{M,\gamma_1}(t)=  \lim_{N\to\infty} X^{N}(0)+\sum_{j : \gamma_1+\tilde \rho_j>0}  \int_0^t \lambda'_j \left(\tilde {\mathcal K}^{M,\gamma_1}(t),\tilde X^{M,\gamma_1}(s)\right) D^0\left(v'_{\cdot j}-v_{\cdot j}\right) \dd s \\
&\qquad\qquad\quad+\sum_{j : \gamma_1+\tilde \rho_j=0 } R_j\left( \int_0^t \lambda'_j \left(\tilde {\mathcal K}^{M,\gamma_1}(t), \tilde X^{M,\gamma_1}(s)\right) D^{\gamma_1+\tilde \rho_j}\left(v'_{\cdot j}-v_{\cdot j}\right) \dd s \right)  \\
&\left\{\begin{array}{cclr}
\dot{\tilde {\mathcal K}}^{M,\gamma_1} (t) &=& 0   & t\notin  \left\{ t_i\right\}_{i\in\mathbb N}\\
\tilde {\mathcal K}^{M,\gamma_1} (t) & \sim& \eta_{M} \left(\cdot\left| \tilde {\mathcal K}^{M,\gamma_1} (t^-)\right.\right) & t\in\left\{ t_i\right\}_{i\in\mathbb N} 
\end{array}
\right.
\end{align*}
where $\tilde {\mathcal K}^{M,\gamma_1} (0)=\mathcal K$. 
The above process can be seen as a variants of the hybrid model \eqref{eq. reduced model at the first time scale}, where the model parameter is perturbed by some artificial noise at time points $\left\{ t_i\right\}_{i\in\mathbb N}$.
Also, we define the observation of the process by
\begin{equation*}
	\tilde Y^{M,\gamma_1}(t_i) = h\left(\tilde X^{M,\gamma_1}(t_i)\right) + W(t_i)
\end{equation*}
and $\tilde {\mathcal Y}^{M,\gamma_1}_{t_i}$ be the $\sigma$-algebra generated by the above readouts up to the time $t_i$. 
For a bounded measurable function $\phi$, let $\tilde \pi ^{M,\gamma_1}_{t_i}(\phi)\triangleq \mathbb E_{\mathbb P} \left[ \left(\tilde {\mathcal K}^{M,\gamma_1}(t_i^-), \tilde X^{M,\gamma_1}(t_i)  \right) \left| \tilde {\mathcal Y}^{M,\gamma_1}_{t_i} \right. \right]$ and $\hat f^{M}_{\phi,t}$ be a mapping such that 
\begin{equation*}
	\hat f^{M}_{\phi,t_i} \left( \tilde {\mathcal Y}^{M,\gamma_1}_{1:i} \right) = \tilde \pi ^{M,\gamma_1}_{t_i}(\phi)
\end{equation*}
where $\tilde {\mathcal Y}^{M,\gamma_1}_{1:i}=\left( \tilde {\mathcal Y}^{M,\gamma_1}_{t_1},\dots, \tilde {\mathcal Y}^{M,\gamma_1}_{t_i} \right)$.
Obviously, the constructed filter $\bar \pi^{N,\gamma_1}_{M,t_i}(\phi)$ is an SIR particle filter for the above system, and by \cite[Corollary 2.4.4]{crisan2001particle}, the filter $\bar \pi^{N,\gamma_1}_{M,t_i}(\phi)$ converges almost surely to $\hat f^{M}_{\phi,t_i} \left( {\mathcal Y}^{N,\gamma_1}_{1:i} \right)$ as $M\to\infty$ for any fixed $N$.
This fact together with \cref{pro. fang} suggests that to prove the main theorem, we only need to check $\hat f^{M}_{\phi,t_i} \left(  {\mathcal Y}^{N,\gamma_1}_{1:i} \right) \to \hat f_{\phi, t_i} \left(  {\mathcal Y}^{N,\gamma_1}_{1:i} \right)  $ in probability as $M\to\infty$ for any fixed $N$.
In the following, we will show the result by borrowing \cite[Lemma 2.37]{del2000branching} which requires the transition kernel to be globally Lipschitz.

In our setting, the transition kernel of the hybrid model is not necessarily globally Lipschitz as the propensity is only locally Lipschitz (see \cref{cond. Lipschitz continuity of propensities}). 
Therefore, we cannot borrow \cite[Lemma 2.37]{del2000branching} directly. 
Instead, we look at the stopped process, whose transition kernel is then globally Lipschitz, and show the filters for such stopped processes converges by using \cite[Lemma 2.37]{del2000branching}.
Finally, by passing the stopping time to infinity, we can show the final result. 

We first show that the transition kernel of the stopped hybrid process is globally Lipschitz.
Let us term $\tau_c$ as the first passage time of the process $X^{\gamma_1}(t)$ of existing a compact region $\{x| \left\|x\right\|_2\leq c\}$ and $\tau^M_c$ as the first passage time of $\tilde X^{M,\gamma_1}(t)$ of existing the same compact region.
According to \cite[Lemma 10.2]{bain2008fundamentals}, for any $i\in\mathbb N_{>0}$ and $y\in\mathbb R^{m\times i}$, there hold
\begin{align}
	\hat f_{\phi, t_i}(y) &= \frac{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\mathcal K, X^{\gamma_1}(t_j)\right) \phi \left(\mathcal K, X^{\gamma_1}(t_i)\right)  \right]}{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\mathcal K, X^{\gamma_1}(t_j)\right) \right]},  \label{eq. Kallianpur-Striebel formula hybrid model} \\
	\hat f^M_{\phi, t_i}(y) &= \frac{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\tilde {\mathcal K}^{M,\gamma_1}(t_j), \tilde X^{M,\gamma_1}(t_j) \right) \phi \left(\tilde {\mathcal K}^{M,\gamma_1}(t_i), \tilde X^{M, \gamma_1}(t_i)\right)  \right]}{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\tilde {\mathcal K}^{M,\gamma_1}(t_j), \tilde X^{M,\gamma_1}(t_j) \right) \right]}  \label{eq. Kallianpur-Striebel formula auxiliary model}. 
\end{align}
Then for any $i\in\mathbb N_{>0}$ and $y\in\mathbb R^{m\times i}$, we define filters for stopped processes as follows. 
\begin{align}
\hat f^c_{\phi, t_i}(y) &\triangleq  \frac{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\mathcal K, X^{\gamma_1}(t_j\wedge \tau_c)\right) \phi \left(\mathcal K, X^{\gamma_1}(t_i\wedge \tau_c)\right)  \right]}{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\mathcal K, X^{\gamma_1}(t_j\wedge \tau_c)\right) \right]},  \label{eq. Kallianpur-Striebel formula hybrid model stopping time} \\
\hat f^{c,M}_{\phi, t_i}(y) &\triangleq \frac{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\tilde {\mathcal K}^{M,\gamma_1}(t_j), \tilde X^{M,\gamma_1}(t_j\wedge \tau^{M}_c) \right) \phi \left(\tilde {\mathcal K}^{M,\gamma_1}(t_i), \tilde X^{M, \gamma_1}(t_i\wedge \tau_c^M)\right)  \right]}{\mathbb E_{\mathbb P}\left[ \prod_{j=1}^i \ell_y\left(\tilde {\mathcal K}^{M,\gamma_1}(t_j), \tilde X^{M,\gamma_1}(t_j\wedge \tau^M_c) \right) \right]}  \label{eq. Kallianpur-Striebel formula auxiliary model stopping time}. 
\end{align}


\textcolor{red}{It is not easy to show the sensitivity analysis of a stopped process.}

\begin{lemma}{\label{lemma convergence of filters for stopped processes}}
	If \cref{assumption convergence of the initial condition}, \cref{cond. conditions on the artificial noise 1} \cref{cond. Lipschitz continuity of propensities} hold, then for any $c>0$, $i\in\mathbb N_{>0}$, and $y\in\mathbb R^{m\times i}$,  there holds $\lim_{M\to\infty}\hat f^{c,M}_{\phi, t_i}(y)  \to \hat f^c_{\phi, t_i}(y) $ almost surely.
\end{lemma}

\begin{proof}
	We first show that the transition kernel of the stopped hybrid process, i.e., $$\mathcal K^{c}_{t}(z,A)\triangleq \mathbb P \left( \left(\mathcal K, X^{\gamma_1}(t\wedge \tau_c)  \right) \in A \left| \left(\mathcal K, X^{\gamma_1}(0)  \right) =z \right.\right) \qquad \forall z \in \Theta \times \mathbb R^{n}_{\geq 0} \text{ and } \forall A\subset \mathbb R, $$
	maps the set of globally Lipschitz function to its self. To do the sensitivity analysis, we follow the literature \cite{anderson2012efficient} to construct two highly coupled processes $(\hat{\mathcal K}_1, \hat X_1(t))$ and $(\hat{\mathcal K}_2, \hat X_2(t))$ as follows.
	\begin{align}
	&\hat X_1(t) \notag \\%\label{eq. K1 and X1}  \\
	&=\lim_{N\to \infty} X^{N}(0) + \sum_{j : \gamma_1+\tilde \rho_j>0} \int_0^t \lambda'_j( \hat{\mathcal K}_1, \hat {X}_1(s))  D^{\gamma_1+\tilde \rho_j}\left(v'_{\cdot j}-v_{\cdot j}\right)\dd s \notag   \\
	&\quad +\sum_{j : \gamma_1+\tilde \rho_j=0 } R^{(0)}_j\left( \int_0^t \lambda'_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\dd s \right) D^0\left(v'_{\cdot j}-v_{\cdot j}\right) \notag \\
	&\quad + \sum_{j : \gamma_1+\tilde \rho_j=0 } R^{(1)}_j\left( \int_0^t \lambda'_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda'_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s)) \dd s \right) D^0\left(v'_{\cdot j}-v_{\cdot j}\right) \notag \\
	&\hat X_2(t) \notag \\ % \label{eq. K2 and X2} \\
	&=\lim_{N\to \infty} X^{N}(0) + \sum_{j : \gamma_1+\tilde \rho_j>0} \int_0^t \lambda'_j( \hat{\mathcal K}_2, \hat {X}_2(s))  D^{\gamma_1+\tilde \rho_j}\left(v'_{\cdot j}-v_{\cdot j}\right)\dd s \notag   \\
	&\quad +\sum_{j : \gamma_1+\tilde \rho_j=0 } R^{(0)}_j\left( \int_0^t \lambda'_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\dd s \right) D^0\left(v'_{\cdot j}-v_{\cdot j}\right) \notag \\
	&\quad + \sum_{j : \gamma_1+\tilde \rho_j=0 } R^{(2)}_j\left( \int_0^t \lambda'_j (\hat{\mathcal K}_2, \hat X_2(s))- \lambda'_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s)) \dd s \right) D^0\left(v'_{\cdot j}-v_{\cdot j}\right) \notag 
	\end{align}
	where $\left(\hat{\mathcal K}_1, \hat X_1(0)\right)$ and $\left(\hat{\mathcal K}_2,\hat X_2(0)\right)$ have the same law as $(\mathcal K, X(0))$, and $\{R^{(0)}_{j}(\cdot)\}_{j}$, $\{R^{(1)}_{j}(\cdot)\}_{j}$, and $\{R^{(2)}_{j}(\cdot)\}_{j}$ are mutually independent, unit rate Poisson processes.
	Obviously, the processes $\left(\hat{\mathcal K}_1, \hat X_1(\cdot)\right)$, $\left(\hat{\mathcal K}_2,\hat X_2(\cdot)\right)$ and $(\mathcal K, X(\cdot))$ have the same law under the natural probability measure. 
    
    According to the above equations we have that 
    \begin{align*}
    &\left\| \hat X_1(t)-\hat X_2(t) \right\|_2\\
    &\leq \left\| \hat X_1(0)-\hat X_2(0) \right\|_2+ \sum_{j=1}^{r}  \left\|\int_0^t \left(\lambda_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\right)\zeta_j \mathbbold{1}_{\{\delta_j=0\}}\dd s\right\|_2\\
    & \quad+ \sum_{j=1}^{r}  R^{(1)}_j\left( \int_0^t \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s)) \dd s \right) \left\|\zeta_j \mathbbold{1}_{\{\delta_j=1\}} \right\|_2 \\
    &\quad+ \sum_{j=1}^{r} R^{(2)}_j\left( \int_0^t \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))- \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s)) \dd s \right) \left\| \zeta_j \mathbbold{1}_{\{\delta_j=1\}} \right\|_2
    \end{align*} 
	
	
	~
	~
	
	
\end{proof}



~

~




~

~




\newpage


One method to do the sensitivity analysis is to construct auxiliary random processes that have the same laws as the nominal and perturbed process and, meanwhile, are highly coupled \cite{anderson2012efficient} (also see \cite{gupta2013unbiased}). 
Following the method in \cite{anderson2012efficient}, we term $(\hat{\mathcal K}_1, \hat X_1(t))$ and $(\hat{\mathcal K}_2, \hat X_2(t))$ as two stochastic processes satisfying

where $\left(\hat{\mathcal K}_1, \hat X_1(0)\right)$ and $\left(\hat{\mathcal K}_2,\hat X_2(0)\right)$ have the same law as $(\mathcal K, X(0))$, and $\{R^{(0)}_{j}(\cdot)\}_{j}$, $\{R^{(1)}_{j}(\cdot)\}_{j}$, and $\{R^{(2)}_{j}(\cdot)\}_{j}$ are mutually independent, unit rate Poisson processes.
Also, we set the above Poisson processes and system parameters to be independent of  $(\mathcal K, X(\cdot))$ (see \eqref{eq. the hybrid crn}) and the observation noises, so that the above processes are independent of $Y_c(\cdot)$ and $Y_d(\cdot)$. 
Obviously, the processes $\left(\hat{\mathcal K}_1, \hat X_1(\cdot)\right)$, $\left(\hat{\mathcal K}_2,\hat X_2(\cdot)\right)$ and $(\mathcal K, X(\cdot))$ have the same law under the natural probability measure. 
The advantage of the above constructions is that the constructed processes are highly correlated and satisfy the following results.

\begin{proposition}{\label{prop. sensitivity}}
	Let $\left(\hat{\mathcal K}_1, \hat X_1(t)\right)$ and $\left(\hat{\mathcal K}_2, \hat X_2(t)\right)$ satisfy \eqref{eq. K1 and X1} and \eqref{eq. K2 and X2}, respectively.
	If \eqref{eq. assumption infinite explosion time} and \cref{cond. global Lipschitz continuity of propensities} hold, then for any $t>0$, $\kappa_1,\kappa_2\in\Theta$, and $x_1, x_2 \in\mathbb{X}$, there exist time dependent scalars $C_{1,t}$ and $C_{2,t}$, such that 
	\begin{align*}
		&\mathbb E_{\mathbb P} \left[  
		   \left\| \hat X_1(t)- \hat X_2(t)\right\|_{2} 
		   \Big| 
		   \hat{\mathcal K}_1=\kappa_1, ~\hat{\mathcal K}_2=\kappa_2,~ \hat X_1(0)=x_1,~ \hat X_2(0)=x_2	   
		\right] \\
		&\leq C_{1,t} \left(\left\|\kappa_1-\kappa_2\right\|_2+ \left\|x_1-x_2\right\|_2 \right).
	\end{align*}
%	and
%	\begin{align*}
%	&\mathbb E_{\mathbb P} \left[  
%	\left\| \hat X_1(t)- \hat X_2(t)\right\|^2_{2} 
%	\Big| 
%    \hat{\mathcal K}_1=\kappa_1, ~\hat{\mathcal K}_2=\kappa_2,~ \hat X_1(0)=x_1,~ \hat X_2(0)=x_2
%	\right] \\
%	&\leq C_{2,t}  \left(\left\|\kappa_1-\kappa_2\right\|_2+ \left\|x_1-x_2\right\|_2 \right)
%	\end{align*}
\end{proposition}

\begin{proof}
	By subtracting \eqref{eq. K2 and X2} from \eqref{eq. K1 and X1} and taking the Euclidean norm on both sides, we have that 
	\begin{align*}
		&\left\| \hat X_1(t)-\hat X_2(t) \right\|_2\\
		&\leq \left\| \hat X_1(0)-\hat X_2(0) \right\|_2+ \sum_{j=1}^{r}  \left\|\int_0^t \left(\lambda_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\right)\zeta_j \mathbbold{1}_{\{\delta_j=0\}}\dd s\right\|_2\\
		& \quad+ \sum_{j=1}^{r}  R^{(1)}_j\left( \int_0^t \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s)) \dd s \right) \left\|\zeta_j \mathbbold{1}_{\{\delta_j=1\}} \right\|_2 \\
		&\quad+ \sum_{j=1}^{r} R^{(2)}_j\left( \int_0^t \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))- \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s)) \dd s \right) \left\| \zeta_j \mathbbold{1}_{\{\delta_j=1\}} \right\|_2
	\end{align*} 
	Let us denote an event $A\triangleq\left\{ \hat{\mathcal K}_1=\kappa_1, ~\hat{\mathcal K}_2=\kappa_2,~ \hat X_1(0)=x_1,~ \hat X_2(0)=x_2\right\}$, and a conditional expectation $\epsilon_1(t)\triangleq\mathbb E_{\mathbb P} \left[  
	\left\| \hat X_1(t)- \hat X_2(t)\right\|_{2} 
	\Big| 
	A
	\right]$.
	Then, by taking the conditional expectation on both sides of the above inequality and considering \cref{cond. global Lipschitz continuity of propensities}, we have that 
	\begin{equation*}
		\epsilon_1(t) \leq \left\|x_1-x_2\right\|_2+ r C_{\lambda}\left(\max_{j\in\{1,\dots,r\}} \left\| \zeta_j\right\|_2\right) 
		\left( t \|\kappa_1-\kappa_2\|_2 +\int_0^{t} \epsilon_1(s)  \dd s \right)
	\end{equation*}
	for any $ t\leq \sup\{s|\epsilon_1(s)<\infty \}$, which, together with Gronwall's inequality, proves the first inequality of this proposition. 
\end{proof}
%	Let $\epsilon_2(t)\triangleq\mathbb E_{\mathbb P} \left[  
%	\left\| \hat X_1(t)- \hat X_2(t)\right\|^2_{2} 
%	\Big| 
%	A  
%	\right]$.
%    By \eqref{eq. K2 and X2}, \eqref{eq. K1 and X1} and \eqref{eq. assumption infinite explosion time}, we can obtain that for any $t\leq \sup\{s|\epsilon_2(s)<\infty \}$, there holds
%	\begin{align*}
%	 &\epsilon_2(t) \\
%	 &=  \sum_{j=1}^r\int_0^{t} \mathbb E_{\mathbb P} \left[  
%	2\left(\lambda_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\right) \left( \hat X_1(t)- \hat X_2(t)\right)^{\top}\zeta_j \mathbbold{1}_{\{\delta_j=0\}}
%	\Big| 
%	A
%	\right] \dd s \\
%	&\quad + \sum_{j=1}^r \int_0^{t} \mathbb E_{\mathbb P} \Big[  
%	\mathbbold{1}_{\{\delta_j=1\}}\left( \|\hat X_1(s)- \hat X_2(s)+\zeta_j\|^2_2-\|\hat X_1(s)- \hat X_2(s)\|_2^2\right)\\
%	&\qquad\qquad\qquad\qquad\qquad
%	\times\left(\lambda_j (\hat{\mathcal K}_1, \hat X_1(s))- \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\right)
%	\Big| 
%	A
%	\Big] \dd s \\
%	&\quad + \sum_{j=1}^r \int_0^{t} \mathbb E_{\mathbb P} \Big[  
%	\mathbbold{1}_{\{\delta_j=1\}}\left( \|\hat X_1(s)- \hat X_2(s)-\zeta_j\|^2_2-\|\hat X_1(s)- \hat X_2(s)\|_2^2\right)\\
%	&\qquad\qquad\qquad\qquad\qquad
%	\times\left(\lambda_j (\hat{\mathcal K}_2, \hat X_2(s))- \lambda_j (\hat{\mathcal K}_1, \hat X_1(s))\wedge \lambda_j (\hat{\mathcal K}_2, \hat X_2(s))\right)
%	\Big| 
%	A
%	\Big] \dd s. 
%	\end{align*}
%	Then, for any $t\leq \sup\{s|\epsilon_2(s)<\infty \}$, we can show by \cref{cond. global Lipschitz continuity of propensities} that
%	\begin{align*}
%		\epsilon_2(t) \leq& 2C_{\lambda}\left(\max_{j\in\{1,\dots,r\}}\left\| \zeta_j\right\|_2\right) 
%		\left(\|\kappa_1-\kappa_2\|_2 \int_0^t \epsilon_1(s) \dd s +\int_0^{t} \epsilon_2(s)  \dd s \right) \\
%		&+r C_{\lambda}\left(\max_{j\in\{1,\dots,r\}} \zeta_j^{\top}\zeta_j\right) 
%		\left( t\|\kappa_1-\kappa_2\|_2  +\int_0^{t} \epsilon_1(s)  \dd s \right)
%	\end{align*}
%	which, together with the compactness of $\Theta$, the first inequality of the proposition, and Gronwall's inequality, proves the second inequality.c


Notably, the mean squared error of $\hat X_1(t)$ and $\hat X_2(t)$ is of the order $O\left(\|k_1-k_2\|\right)$ rather than $O\left(\|k_1-k_2\|^2\right)$.
It is because we consider Poisson noise in this paper, and the mean and variance of a Poisson random variable are the same.  


\section{The proof of \cref{pro. verify the second contion of del Moral's lemma}}

\begin{proof}[The proof of \cref{pro. verify the second contion of del Moral's lemma}]
	Since $(\mathcal K, X(\cdot))$, $\left(\hat{\mathcal K}_1,  \hat X_1(\cdot)\right)$, and $\left(\hat{\mathcal K}_2,  \hat X_2(\cdot)\right)$ have the same law, we can write
	\begin{align*}
	&\Big| \mathbb E_{\mathbb P}\left[
	f\left(\mathcal K, X(t_i)\right) \left| \mathcal K=\kappa_1, X(0)=x_1\right.
	\right]
	-
	\mathbb E_{\mathbb P}\left[
	f\left(\mathcal K, X(t_i)\right) \left| \mathcal K=\kappa_2, X(0)=x_2\right.
	\right]
	\Big| \\
	&=\Big|\mathbb E_{\mathbb P}\left[
	f\left( \hat {\mathcal K}_1, \hat X_1(t_i)\right) \left| \hat{\mathcal K}_1 =\kappa_1, \hat X_1(0)=x_1\right.
	\right] \\
	&\qquad
	-
	\mathbb E_{\mathbb P}\left[
	f\left(\hat {\mathcal K}_2, \hat X_2(t_i)\right) \left| \hat{\mathcal K}_2=\kappa_2, \hat X_2 (0)=x_2\right.
	\right]
	\Big| \\
	&=
	\left| \mathbb E_{\mathbb P}\left[
     f\left( \hat {\mathcal K}_1, \hat X_1(t_i)\right)-f\left(\hat {\mathcal K}_2, \hat X_2(t_i)\right)  \left| \hat{\mathcal K}_1 =\kappa_1, \hat{\mathcal K}_2=\kappa_2, \hat X_1(0)=x_1, \hat X_2 (0)=x_2\right.
	\right] 	\right|  \\
	&\leq
    \mathbb E_{\mathbb P}\left[
	\left| f\left( \hat {\mathcal K}_1, \hat X_1(t_i)\right)-f\left(\hat {\mathcal K}_2, \hat X_2(t_i)\right)	\right|   \left| \hat{\mathcal K}_1 =\kappa_1, \hat{\mathcal K}_2=\kappa_2, \hat X_1(0)=x_1, \hat X_2 (0)=x_2\right.
	\right] 
	\end{align*}
	where the forth line follows from the fact that the laws of $\left(\mathcal K_1, \hat X_1(\cdot)\right)$ and $\left(\mathcal K_2, \hat X_2(\cdot)\right)$ are irrelevant to each other's initial conditions, and the last line follows from Jensen's inequality.
	Therefore, this proposition follows immediately from \cref{pro. the same law of X and hat X} and the Lipschitz continuity of the function $f$.
\end{proof}


\section{Proof for the continuous-time cases}
We define analogs to $Z_c(t)$ using $\hat{X}_1(\cdot)$ and $\hat X_2(\cdot)$.
For $\ell=1,2$, we denote
\begin{equation*}
\hat Z_{\ell, c}  (t)\triangleq \exp\left( \int_{0}^{t} h^{\top}\left(\hat X_\ell(s)\right) \dd Y_c(s) - \frac{1}{2} \int_0^{t} \left\|h\left(\hat X_\ell (s)\right)\right\|^2_2 \dd s \right), 
\qquad \forall t>0,
\end{equation*}

\begin{proposition}{\label{pro. the same law of X and hat X}}
	Conditioned on $\mathcal Y_{c,t}$, random variables $\left(\hat X_{\ell}(\cdot), \hat Z_{\ell,c}(\cdot)\right)$ ($\ell=1,2$) under $\mathbb P$ have the same conditional law as $\left( X(\cdot),  Z_{c}(\cdot)\right)$ under  $\mathbb Q_c$.
\end{proposition}
\begin{proof}
	It follows straightforwardly from the definition.
\end{proof}

Therefore, we can also conclude that 
\begin{align}{\label{eq bar phi hat K hat X}}
\bar \phi_{\tau,t}(\kappa,x, y) 
= & \mathbb E_{\mathbb P}\left[ \frac{\hat Z_{c,\ell}(t)}{\hat Z_{c,\ell}(\tau)} \phi(\hat{\mathcal K}_{\ell}, \hat X_{\ell}(t))\left| \hat{\mathcal K}_{\ell} =\kappa, \hat X_{\ell}(\tau)=x, Y_{c,\tau:t}=y  \right. \right]
\end{align}
for $\ell=1,2$.

\begin{proof}[The proof of \cref{pro continuous-time inequality}]
	To simplify the notations, let us first denote an event 
	$A\triangleq\left\{ \hat{\mathcal K}_1=\kappa_1, ~\hat{\mathcal K}_2=\kappa_2,~ \hat X_1(0)=x_1,~ \hat X_2(0)=x_2\right\}$.
	By \eqref{eq bar phi hat K hat X}, we can show that 
	\begin{align*}
		&\text{The forth square root of the left hand side of \eqref{eq. continuous-time inequality}}\\
		&= 	\sqrt[4]{\mathbb E_{\mathbb P} \left[\left( \mathbb E_{\mathbb P}\left[ \left. \frac{\hat Z_{1,c}(t)}{\hat Z_{1,c}(\tau)} \phi\left(\hat{\mathcal K}_1, \hat X_1(t)\right) \right| \mathcal Y_{c,t} \vee A  \right] 
		- \mathbb E_{\mathbb P}\left[ \left.  \frac{\hat Z_{2, c}(t)}{\hat Z_{2,c}(\tau)} \phi\left(\hat{\mathcal K}_2, \hat X_2 (t)\right) \right| \mathcal Y_{c,t} \vee A \right] 
		\right)^4 \right] } \notag\\
		&\leq \sqrt[4]{\mathbb E_{\mathbb P} \left[ 
		\left.	
		\left( 
		\frac{\hat Z_{1,c}(t)}{\hat Z_{1,c}(\tau)} \phi\left(\hat{\mathcal K}_1, \hat X_1(t)\right) 
		- 
	    \frac{\hat Z_{2, c}(t)}{\hat Z_{2,c}(\tau)} \phi\left(\hat{\mathcal K}_2, \hat X_2 (t)\right) 
	    \right)^4
	    \right| A
	    \right]} \\
        &\leq \sqrt[4]{\mathbb E_{\mathbb P} \left[
        	\left.\left( 
        	\left(\frac{\hat Z_{1,c}(t)}{\hat Z_{1,c}(\tau)} 
        	- 
        	\frac{\hat Z_{2, c}(t)}{\hat Z_{2,c}(\tau)}\right)
        	\phi\left(\hat{\mathcal K}_1, \hat X_1(t)\right)   
        	\right)^4
        	 \right| A
        	\right]}
             \\
         &\qquad +
            \sqrt[4]{\mathbb E_{\mathbb P} \left[ 
            \left.
           \left(\frac{\hat Z_{2,c}(t)}{\hat Z_{2,c}(\tau)} \right)^4
        	\left(\phi\left(\hat{\mathcal K}_1, \hat X_1(t)\right)   - \phi\left(\hat{\mathcal K}_2, \hat X_2(t)\right)   \right)^4
        	 \right| A
        	\right]} \\
        &\leq 8\| \phi\|_{\infty}^4e^{10\|h \|_{\infty}^2(t-\tau)}\sqrt[4]{\mathbb E_{\mathbb P} \left[
        	\left. 
        	e^{4\|h\|_{\infty}\int_\tau^t \left|h\left(\hat X_1(s)\right)-h\left(\hat X_2(s)\right)\right|\dd s}
        	-1
        	\right| A
        	\right]} \\
        & \qquad + 8\| \phi\|_{\infty}^3e^{12\|h \|_{\infty}^2(t-\tau)}
        \sqrt[4]{\mathbb E_{\mathbb P} \left[
        	\left. 
        	\left|\phi\left(\hat{\mathcal K}_1, \hat X_1(t)\right)   - \phi\left(\hat{\mathcal K}_2, \hat X_2(t)\right)   \right|
        	\right| A
        	\right]}      
	\end{align*}
\end{proof}
where the third line follows from Jensen's inequality and the law of total expectation, the forth line follows from the triangle inequality, and the last inequality follows from the independence between $\left(\mathcal K, \hat X_\ell (\cdot)\right)$ (for $\ell=1$ or $2$) and the observation noise $B(\cdot)$.
Finally, by applying the boundedness of $h$, the Lipschitz continuity of $\phi$ and $h$, and \cref{prop. sensitivity} to the above formulas, we can prove the result. 

